Arithmetical Characterizations of Two Intuitionistic Logical Principles

This paper investigates the role of negation in arithmetic by analyzing subsystems based on subminimal logic. We introduce NA^PR, a system of subminimal arithmetic equipped with all primitive recursive functions, and answer the following four questions: (1) Can we develop reasonable arithmetic within NA^PR? (2) Can we characterize logical rules Absorption of Negation (An) and Ex Falso Quodlibet (ECQ) by arithmetical principles? (3) Are there strict differences in deductive power among NA^PR, MA^PR, and HA? (4) Do MA^PR and MA, and NA^PR and NA have a similar mutual interpretability relationship as HA? We show the following: First, Heyting Arithmetic (HA) is shown to be a conservative extension of NA^PR for positive formulas. Based on NA^PR, we prove that (ECQ) is equivalent to the definability of disjunction, and that (An) is equivalent to a variant of the least number principle. Furthermore, using the constant domain neighbourhood semantics, we show that the systems NA^PR, MA^PR (written as NA^PR+(An)) and HA (written as NA^PR+(An)+(ECQ)) form a strictly increasing hierarchy of strength. Finally, we demonstrate the essential role of primitive recursive functions in weak arithmetic using classical countermodels.

==> eptcsdata.tex <==
\providecommand{\firstpage}{21}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.3}{10.4204/EPTCS.455.3}}

